TrimLLM: Progressive Layer Dropping for Domain-Specific LLMs

Specializing large language models (LLMs) for local deployment in domain-specific use cases is necessary for strong performance while meeting latency and privacy constraints. However, conventional task-specific adaptation approaches do not show simultaneous memory saving and inference speedup at deployment time. Practical compression techniques like quantization and pruning require dedicated hardware or kernel support to achieve measured inference speedup. We develop TrimLLM based on the layer-wise specialization phenomenon we empirically observed and verified on contemporary LLMs. TrimLLM reduces the depth of LLMs via progressive layer dropping. We show it retains LLMs' capacity in specific domains and achieves inference speedup irrespective of hardware and deep learning frameworks. We evaluated TrimLLM on LLMs of various sizes for inference; models adapted on medical, legal, and financial datasets all demonstrate $2.1-5.7\times$ inference speedup on consumer GPUs and up to $3.1\times$ speedup on A100 when compared to state-of-the-art model compression algorithms, with no loss in accuracy at 50$\sim$60\% model compression ratio.

==> tables/performance_degradation_teaser.tex <==
\begin{table*}
\centering
\small
\label{tab:perf_teaser}
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\text{model}                                                      & \text{SciQ}        & \text{PIQA}          & \text{HellaSwag}     & \text{OpenBookQA}   & \text{ARC-easy}         & \text{ARC-challenge}         \\ 
\midrule
\text{w/o fine-tuning (100\%)}                                 & 89.7 & 77.4 & 56.4 & 28.2 & 67.4 & 38.2 \\ 
\midrule
\text{SciQ specialized (40\%)} & \textbf{92.8} & 61.5 & 50.5 & 19.4 & 56.0 & 22.5 \\ 
\bottomrule
\end{tabular}
\caption{
Performance of SciQ-specialized LLaMA-7B on other QA benchmarks, which provides empirical evidence that layers containing domain kowledge for other tasks are dropped and those for SciQ are kept. The percentage in parenthesis indicates the percentage of total parameters remained in the specialized model.
}
%\vspace{-0.5\baselineskip}
\end{table*}


==> tables/quantization_pruning_layerdrop_inference.tex <==
\begin{table*}[t]
\centering
\caption{
Deployment-time model inference overhead breakdown (LLaMA-7B, on single V100 GPU, sequence length 512 , batch size 1). The Overhead entry refers to the overhead of running the corresponding model compression algorithm after fine-tuning. The Final Mem entry refers to the ratio of final compressed model size versus the original model size in memory.
}
\small
\label{tab:v100_quantization_pruning_layerdrop_inference}
\begin{tabular}{c|c|c|c}
\toprule
\text{Techniques}                                                      & \text{Overhead (s)}        & \text{Inference Throughput (tokens/s)} & \text{Final Mem}         \\ 
\midrule
\text{FP16}  & \text{N/A} & 16.6 & $100\%$ \\ 
\midrule
\text{LLM.int8()}                                 & 57.3 & 4.1 & $\geq50\%$ \\ 
\text{GPTQ-int4} & 371.5 & 7.2 & $>25\%$ \\ 
\text{AWQ-int4} & 542.9 & 29.3 & $>25\%$ \\ 
\midrule
\text{Sparse-GPT (2:4)} & 215.4 & 21.2 & $100\%$ \\ 
\text{Masked Pruning} & 253.2 & 17.7 & $100\%$ \\ 
\text{Activation-based Pruning} & 0.54 & 16.1 & $100\%$ \\ 
\midrule
\text{Sapling (40\%)} & \text{N/A} & \textbf{34.9} & $\geq40\%$ \\ 
\bottomrule
\end{tabular}
%\vspace{-2\baselineskip}
\end{table*}
